Exploratory numerical experiments with a macroscopic theory of interfacial interactions

Phenomenological theories of interfacial interactions have targeted terrestrial applications since long time and their exploitation has inspired our research programme to build up a macroscopic theory of gas-surface interactions targeting the complex phenomenology of hypersonic reentry flows as alternative to standard methods based on accommodation coefficients. The objective of this paper is the description of methods employed and results achieved in an exploratory study, that is, the unsteady heat transfer between two solids in contact with and without interface. It is a simple numerical-demonstrator test case designed to facilitate quick numerical calculations and to bring forth already sufficiently meaningful aspects relevant to thermal protection due to the formation of the interface. The paper begins with a brief introduction on the subject matter and a review of relevant literature. Then the case is considered in which the interface is absent. The importance of tension continuity as boundary condition on the same footing of heat-flux continuity is recognised and the role of the former in governing the establishment of the temperature-difference distribution over the separation surface is explicitly shown. Evidence is given that the standard temperature-continuity boundary condition is just a particular case. Subsequently the case in which the interface is formed between the solids is analysed. The coupling among the heat-transfer equations applicable in the solids and the balance equation for the surface thermodynamic energy formulated in terms of the surface temperature is discussed. Results are illustrated for planar and cylindrical configuration; they show unequivocally that the thermal-protection action of the interface turns out to be driven exclusively by thermophysical properties of the solids and of the interface; accommodation coefficients are not needed.

==> local.tex <==
% fonts declarations
%
%\DeclareFontEncoding{OT1}{}{}
%\renewcommand{\familydefault}{ptm}   % times roman is the default font
%
\newcommand\yinitfamily{\usefont{U}{yinit}{m}{n}}     % yinit 
\DeclareTextFontCommand{\textyinit}{\yinitfamily}

\definecolor{halfgreen}{rgb}{0,0.5,0}
% symbols

\newcommand{\jr}      {j=1,\cdots,s}                             % j range
\newcommand{\ir}      {i=1,\cdots,n}                             % i range
\newcommand{\kr}      {k=1,\cdots,r}                             % k range
\newcommand{\isr}     {i=n-s+1,\cdots,n}                         % i subrange
\newcommand{\dr}      {\delta=1,\cdots,\Li}                      % delta range
\newcommand{\id}      {i\delta}                                  % i-component,(delta)-dof
%\newcommand{\id}      {\mbox{\tiny$i\delta$}}                    % i-component,(delta)-dof
\newcommand{\Li}      {\ell_{i}}                                 % dofs of i-component
\newcommand{\sLi}     {\displaystyle \sum_{i=1}^n \Li}           % i-sum of Li
\newcommand{\sid}     {\displaystyle \sum_{i=1}^n\sum_{\delta=1}^{\Li}}
                                                                 % (i,delta)-sum 
%\newcommand{\sid}     {\displaystyle \sum_{i,\delta}}            % (i,delta)-sum 
\newcommand{\dir}     {\parbox[c]{10em}{\centering $\dr$\\$\ir$}}

\newcommand{\R}{\bv{r}}
\newcommand{\Ro}{\R_{\circ}}
%\newcommand{\Ut}       {\mbox{\sffamily \textbf{U}}}              % isotropic (unit) tensor
\newcommand {\GradT}  {\bv{$\nabla$}_{\mbox{\tiny T}}}           % isothermal gradient operator 

\newcommand{\CF}  [1] {\mbox{C\hspace*{-0.1ex}F}_{#1}}           % chemical formula
%\newcommand{\CF}  [1] {\mbox{C}_{#1}}           % chemical formula
\newcommand{\nur} [1] {\nu_{#1}^{\mbox{\tiny (r)}}}              % reactant stoichiometric coefficient
\newcommand{\nup} [1] {\nu_{#1}^{\mbox{\tiny (p)}}}              % product  sotichiometric coefficient
\newcommand{\Kfk}     {\textcolor{halfgreen}{\mbox{\Large$\kappa$}_k^{\mbox{\Tiny f}}}} % forward  reaction constant
\newcommand{\Kbk}   {\textcolor{halfgreen}{\mbox{\Large$\kappa$}_k^{\mbox{\Tiny b}}}} % backward reaction constant
\newcommand{\Kfb}     {\mbox{\Large$\kappa$}^{\mbox{\tiny f,b}}} % forward/backward reaction constant
\newcommand{\Kck}     {K_k^{\mbox{\tiny c}}}                     % equilibrium constant Kc

\newcommand{\hp}      {\textcolor{red}{f_{\id}}}                            % i-delta Helmholtz potential
\newcommand{\Af}  [1] {{\cal A}_{#1}}                            % chemical affinity

%\newcommand{\mf}  [1] {\alpha_{\mbox{\tiny $#1$}}}               % component mass fraction
\newcommand{\mf}  [1] {\alpha_{#1}}                              % component mass fraction
\newcommand{\mof}  [1] {x_{#1}}                              % component molar fraction
%\newcommand{\gv}      {g_{v}}                                    % generic-variable density (unit volume)
\newcommand{\gvp}      {g^{\mbox{\Tiny +}}}                                    % generic-variable density (unit volume)

\newcommand{\V}       {\bv{v}}                                   % velocity vector
%\newcommand{\am}    {\bv{s}}                                   % angular-momentum vector
\newcommand{\am}    {\bv{\mbox{$\frak{s}$}}}          % angular-momentum vector
\newcommand{\amm}       {\bv{\mbox{$\frak{L}$}}}        % intrinsic moment of matter momentum per unit mass
\newcommand{\K}       {\bv{k}}                               % intrinsic moment of matter momentum per unit mass 
\newcommand{\amt}       {\bv{L}}                               % intrinsic moment of matter momentum per unit mass 
\newcommand{\n}       {\bv{n}}                                   % outward normal to a surface
\newcommand{\gvso}    {(\Grad\V)^{\mbox{\hspace*{.1em}\Tiny s}}_{\mbox{\Tiny o}}}
                                                                 % traceless-symmetric part of velocity gradient
\newcommand{\gva}     {(\Grad\V)^{\mbox{\hspace*{.1em}\Tiny a}}} % antisymmetric part of velocity gradient
\newcommand{\kem}     {\frac{\mbox{v}^2}{2}}                     % kinetic energy per unit mass
\newcommand{\me}      {e_{\mbox{\Tiny m}}}                       % matter-energy per unit mass
\newcommand{\eme}     {e_{\mbox{\Tiny em},v}}                    % em-energy per unit volume
\newcommand{\emee}    {\frac{\eo}{2}(E^2+c^2B^2)}                % em-energy per unit volume (explicit)
\newcommand{\gee}    {(g^2 + c^2 b^2) / 2}                % g-energy per unit volume (explicit)
%\newcommand{\s}       {\mbox{\calligra\Large s}}                 % entropy per unit mass
%\newcommand{\s}       {\mbox{\large$\frak{s}$}}                 % entropy per unit mass
\newcommand{\s}       {s}                 % entropy per unit mass
\newcommand{\si}      {\s_{\,i}}                                 % specific entropy i-th component
\newcommand{\Fi}      {\mbox{\boldmath $\EuScript{F}$}_{i}}         % generalized force -> Jmi
\newcommand{\X}   [1] {\mbox{\boldmath $\EuScript{X}$}_{#1}}      % generalized force -> Wi

\newcommand{\Lqi}     {{\mbox{\textbf{\sffamily L}}}_{\mbox{\tiny T}i}}
\newcommand{\Liq}     {{\mbox{\textbf{\sffamily L}}}_{i\mbox{\tiny T}}}
\newcommand{\Lqq}     {{\mbox{\textbf{\sffamily L}}}_{\mbox{\tiny TT}}}
\newcommand{\Lij}     {{\mbox{\textbf{\sffamily L}}}_{ij}}
\newcommand{\Dij}     {\textcolor{halfgreen}{{{\mbox{\textbf{\sffamily D}}}_{ij}}}}
\newcommand{\Dik}     {\textcolor{halfgreen}{{{\mbox{\textbf{\sffamily D}}}_{ik}}}}
\newcommand{\Din}     {\textcolor{halfgreen}{{{\mbox{\textbf{\sffamily D}}}_{in}}}}
\newcommand{\DiT}     {\textcolor{halfgreen}{{{\mbox{\textbf{\sffamily D}}}_{i}^{\mbox{\Tiny T}}}}}
\newcommand{\qm}  [1] {\textcolor{halfgreen}{{\tilde{\mbox{\textbf{\sffamily D}}}_{#1}^{\mbox{\Tiny T}}}(-\B)}}
\newcommand{\DiTt}[1] {\textcolor{halfgreen}{{\tilde{\mbox{\textbf{\sffamily D}}}_{#1}^{\mbox{\Tiny T}}}}}
\newcommand{\Dfl}     {\mbox{\boldmath $\EuScript{D}$}_{ik}}
\newcommand{\Lt}      {\textcolor{halfgreen}{{\mbox{\lambdayb\hspace*{-.4em}$'$}}}}   % thermal conductivity
\newcommand{\Pij}     {{\mbox{\textbf{\sffamily P}}}_{ij}}
\newcommand{\Fmi}     {{\mbox{\textbf{\sffamily F}}_{i}^{\mbox{\Tiny m}}}}
\newcommand{\Fu}      {\textcolor{halfgreen}{{\mbox{\textbf{\sffamily F}}^{\mbox{\Tiny u}}}}}
\newcommand{\Pmi}     {{\mbox{\textbf{\sffamily P}}_{i}^{\mbox{\Tiny m}}}}
\newcommand{\Puj}     {\textcolor{halfgreen}{{\mbox{\textbf{\sffamily P}}_{j}^{\mbox{\Tiny u}}}}}
\newcommand{\Lpj}     {\textcolor{halfgreen}{\mbox{\lambdayb}_{\mbox{\hspace*{-.3em}\Tiny e}j}^{\mbox{\hspace*{-.3em}\Tiny p}}}}
\newcommand{\LeT}     {\textcolor{halfgreen}{\mbox{\lambdayb}_{\mbox{\hspace*{-.3em}\Tiny e}}^{\mbox{\hspace*{-.3em}\Tiny T}}}}
\newcommand{\LuT}     {\textcolor{halfgreen}{\mbox{\lambdayb}_{\mbox{\hspace*{-.3em}\Tiny T}}^{\mbox{\hspace*{-.3em}\Tiny u}}}}
\newcommand{\lkj}     {\textcolor{halfgreen}{l_{kj}}}
\newcommand{\lkk}     {\textcolor{halfgreen}{l_{kk}}}
\newcommand{\lkv}     {\textcolor{halfgreen}{l_{k{\mbox{\scriptsize v}}}}}
\newcommand{\lvk}     {\textcolor{halfgreen}{l_{{\mbox{\scriptsize v}k}}}}
\newcommand{\lvv}     {\textcolor{halfgreen}{l_{\mbox{\scriptsize vv}}}}
\newcommand{\muv}     {\textcolor{halfgreen}{\mbox{\muy\hspace*{-.2em}}_{v}}} % bulk-viscosity coefficient
\newcommand{\mud}     {\textcolor{halfgreen}{\mbox{\muyb\hspace*{-.2em}}}}

\newcommand {\J}  [1] {\bv{J}_{#1}}
\newcommand{\PhiG}    {\bv{$\Phi_{\normalfont\mbox{\Tiny G}}$}}  % generic-variable total flux
\newcommand{\phiG}    {\bv{$\phi_{\normalfont\mbox{\Tiny G}}$}}  % generic-variable total flux
\newcommand{\JG}      {\J{\mbox{\Tiny G}}}                       % generic-variable diffusive flux
\newcommand{\Jm}  [1] {  \textcolor{red}{{\J{\mbox{\scriptsize m}_{#1}}}}  }      % component-mass diffusive flux
\newcommand{\W}   [1] { \textcolor{red}{\bv{C}_{#1}} }                        % component diffusion velocity
\newcommand{\JQ}      {  \textcolor{red}{\J{\mbox{\Tiny Q}}}  }                       % electric-charge diffusive flux
\newcommand{\Jma} [1] {\textcolor{red}{\J{\mbox{\scriptsize m}^{\ast}_{#1}}}}          % element-mass diffusive flux
\newcommand{\T}       {  \textcolor{red}{\mbox{\large \textbf{\taus}}}}       % stress tensor
\newcommand{\Ttr}       {  \textcolor{red}{\mbox{\large $\tilde{\textbf{\taus}}$ }}}       % stress-tensor transpose
%\newcommand{\To}      {  \textcolor{red}{\mathcal{T}}}       % torque tensor
\newcommand{\To}      {  \textcolor{red}{\bv{\mbox{\large$\frak{T}$}}}}       % torque tensor
\newcommand{\nms}     {\textcolor{red}{\mbox{\piy\hspace*{-.2em}}}}         % normal mean stress
\newcommand{\Tso}     {\textcolor{red}{\mbox{{\large\textbf{\taus}}$^{\mbox{\hspace*{.1em}\Tiny s}}_{\mbox{\Tiny o}}$}}}       
                                                                 % traceless symmteric part of stress tensor
\newcommand{\Ta}     {\textcolor{red}{\mbox{{\large\textbf{\taus}}$^{\mbox{\hspace*{.1em}\Tiny a}}$}}}       
                                                                 % antisymmteric part of stress tensor
\newcommand{\Tm}      {\mbox{\large \taus}_{\mbox{\Tiny M}}}     % Maxwell stress tensor
\newcommand{\Tme}     {\eo (\E\E - \frac{1}{2} E^2 \Ut) + \eo c^2 (\B\B - \frac{1}{2} B^2 \Ut)}    % Maxwell stress tensor (explicit)
\newcommand{\Tge}     {\eg (\g\g - \frac{1}{2} g^2 \Ut) + \mug (\bg\bg - \frac{1}{2} b^2 \Ut)} 
\newcommand{\f}       {  \textcolor{red}{\bv{f}} }                                   % body force
\newcommand{\bt}      {  \textcolor{red}{\bv{\mbox{\large$\frak{t}$}}} }                                   % body torque
%\newcommand{\bt}      {  \textcolor{red}{\bv{t}} }                                   % body torque
\newcommand{\Ju}      { \textcolor{red}{\J{\mbox{\Tiny U}}} }                       % internal-energy diffusive flux
\newcommand{\Jur}     {\textcolor{red}{\J{\mbox{\Tiny U}}}}                 % internal-energy diffusive flux - red
\newcommand{\Juid}    {  \textcolor{red}{\J{\mbox{\Tiny U$_{\id}$}}}  }         % i(delta) internal-energy diffusive flux
\newcommand{\Je}      { \textcolor{red}{\J{\mbox{\Tiny E$_{\mbox{\Tiny m}}$}}} }    % matter-energy diffusive flux
\newcommand{\Js}      {\J{\mbox{\Tiny S}}}                       % entropy diffusive flux
\newcommand{\Jq}      {\J{\mbox{\Tiny q}}}                       % heat flux
\newcommand{\Jqa}     { \textcolor{red}{\J{\mbox{\Tiny q}}^{\mbox{\Tiny$'$}}  }}   % heat flux 1
\newcommand{\Jqb}     { \textcolor{red}{\J{\mbox{\Tiny q}}^{\mbox{\Tiny$''$}} }}  % heat flux 2
\newcommand{\Jqc}     { \textcolor{red}{\J{\mbox{\Tiny q}}^{\mbox{\Tiny$'''$}} }} % heat flux 3

\newcommand{\gp }     {\dot{g}}                                  % generic-variable production (unit mass)
\newcommand{\gpv}     {\dot{g}^{\mbox{\Tiny +}}}                              % generic-variable production (unit volume)
\newcommand{\csi} [1] { \textcolor{red}{\dot{\xi}_{#1}} }                     % chemical-reaction rate
\newcommand{\up}      { \textcolor{red}{\dot{u}^{\mbox{\Tiny +}}} }                                % internal-energy production (unit volume)
\newcommand{\upid}    { \textcolor{red}{\dot{u}^{\mbox{\Tiny +}}_{\id}} }                    % i(delta) internal-energy production
\newcommand{\mep}     { \textcolor{red}{\dot{e}^{\mbox{\Tiny +}}_{\mbox{\Tiny m}}} }               % matter-energy production
\newcommand{\kep}     { \textcolor{black}{\dot{e}^{\mbox{\Tiny +}}_{\mbox{\Tiny ke}}} }               % kinetic-energy production
\newcommand{\tep}     { \textcolor{black}{\dot{e}^{\mbox{\Tiny +}}_{\mbox{\Tiny te}}} }               % thermodynamic-energy production
\newcommand{\emep}    {\dot{e}_{\mbox{\Tiny em},v}}              % em-energy production
\newcommand{\enp}     {\;\dot{s}^{\mbox{\Tiny +}}}         % entropy production (unit volume)
%\newcommand{\enp}     {\;\dot{\!\!\mbox{\calligra\Large s}}^{\mbox{\,\Tiny +}}}         % entropy production (unit volume)
\newcommand{\enpo}    {\enp_{\,\mbox{\Tiny 1}}}         % entropy production (unit volume) tensorial order=1
\newcommand{\enpz}    {\enp_{\,\mbox{\Tiny 0}}}         % entropy production (unit volume) tensorial order=0
\newcommand{\vpv}     {\dot{v}_{v}}                              % volume production (unit volume)

\newcommand{\eo}      {\varepsilon_{\mbox{\Tiny 0}}}             % empty-space dielectric constant
\newcommand{\eg}      {\displaystyle \frac{1}{4\pi G}}             % empty-space digravitational constant   :)
\newcommand{\er}      { \mbox{\boldmath $\varepsilon_{\mbox{\Tiny r}}$} }             % dielectric constant
\newcommand{\muo}     {\mu_{\mbox{\Tiny 0}}}                     % empty-space magnetic permittivity
\newcommand{\mug}      {\displaystyle \frac{c^2}{4\pi G}}             % empty-space gravitational permittivity   :)
\newcommand{\mur}     { \mbox{\boldmath $\mu_{\mbox{\Tiny r}}$} }             % magnetic permittivity
\newcommand{\free}    {\textcolor{red}{free}}
\newcommand{\rhocf}   {\rho_{\mbox{\Tiny cf}}}                    % free-electric-charge density
\newcommand{\rhoc}    {\rho_{\mbox{\Tiny c}}}                    % free-electric-charge density
\newcommand{\rhocp}   {\,(\mbox{-}\Dive\Po)\,}                    % polarisation-charge density
\newcommand\cmrfamily{\usefont{T1}{cmr}{m}{n}}    
\DeclareTextFontCommand{\textcmr}{\cmrfamily}
\newcommand{\CDf}     { \textcolor{red}{\textcmr{\bv{\textit{j}}}_{\mbox{\Tiny f}}} }                % free-current density when ptm default
\newcommand{\CD}      { \textcolor{red}{\textcmr{\bv{\textit{j}}}} }                % total current density when ptm default
\newcommand{\CDb}     { \textcmr{\bv{\textit{j}}} }                % total current density when ptm default
\newcommand{\CDp}      {\textcolor{red}{\CD'}}                          % total current density when cmr default
\newcommand{\E}       {\bv{E}}                                   % electric field
\newcommand{\g}       {\bv{g}}                                   % gravitational field
\newcommand{\B}       {\bv{B}}                                   % magnetic field | magnetic induction
\newcommand{\bg}       {\bv{b}}                                   % gravitational induction
\newcommand{\A}       {\bv{A}}                                   % magnetic potential
\newcommand{\M}       {\bv{M}}                                   % magnetization
\newcommand{\Po}      {\bv{P}}                                   % polarization
\newcommand{\D}       {\bv{D}}                                   % electric displacement
\newcommand{\Hi}      {\bv{H}}                                   % magnetic-field intensity
\newcommand{\Le}      {\mbox{\lambday}_{\mbox{\hspace*{-.3em}\Tiny e}}} % electrical conductivity (scalar)
\newcommand{\Let}     {\textcolor{halfgreen}{\mbox{\lambdayb}_{\mbox{\hspace*{-.3em}\Tiny e}}}}     % electrical conductivity (tensor)

  \newcommand{\totene}{\parbox{5em}{\centering total \\ energy}}
  \newcommand{\matene}{\parbox{5em}{\centering \  \\ \textcolor{red}{matter} energy \\ $\rho\me$ }}
  \newcommand{\mateneb}{\parbox{5em}{\centering \  \\ \textbf{\textit{matter}} energy \\ $\rho\me$ }}
  \newcommand{\kinene}{\parbox{5em}{\centering \  \\ kinetic \\ energy \\[1ex] $\rho\;\mbox{v}^{2}/2$ }}
  \newcommand{\intene}{\parbox{8em}{\centering \  \\ thermodynamic \\ energy \\ $\rho u$}}
  \newcommand{\emaene}{\parbox{8em}{\centering \  \\ electromagnetic \\ energy}}

\newcommand{\ic}{\mbox{i}}
\newcommand{\ionc}{\displaystyle \frac{\ic}{c}\,}

\newcommand{\Xe}       {\mbox{\boldmath $\chi_{\mbox{\Tiny e}}$  }}              % electrical-susceptibility tensor
\newcommand{\Xm}       {\mbox{\boldmath $\chi_{\mbox{\Tiny m}}$  }}              % magnetic-susceptibility tensor

\newcommand{\Lgvso} {\textcolor{halfgreen}{\mbox{\sffamily \textbf{L}}}}                  % 
\newcommand{\Lth}   {\textcolor{halfgreen}{\mbox{\hspace{.4em}\lambdayb}}}   % thermal conductivity

\newcommand{\ut}    {u_{\mbox{\scriptsize t}}}
\newcommand{\Tt}    {T_{\mbox{\scriptsize t}}}
\newcommand{\ui}    {u_{\mbox{\scriptsize i}}}
\newcommand{\Ti}    {T_{\mbox{\scriptsize i}}}
\newcommand{\upt}   {\textcolor{red}{\dot{u}^{\mbox{\Tiny +}}_{\mbox{\scriptsize t}}}}             % translational internal-energy production
\newcommand{\upi}   {\textcolor{red}{\dot{u}^{\mbox{\Tiny +}}_{\mbox{\scriptsize i}}}}             % internal      internal-energy production
\newcommand{\Jut}   {\textcolor{red}{\J{\mbox{\Tiny U$_{\mbox{\Tiny t}}$}}}}  % translational internal-energy diffusive flux
\newcommand{\Jui}   {\textcolor{red}{\J{\mbox{\Tiny U$_{\mbox{\Tiny i}}$}}}}  % internal      internal-energy diffusive flux
\newcommand{\Liv}     {l_{\mbox{\scriptsize iv}}}
\newcommand{\Lvi}     {l_{\mbox{\scriptsize vi}}}
\newcommand{\lii}     {l_{\mbox{\scriptsize ii}}}
\newcommand{\Lvv}     {l_{\mbox{\scriptsize vv}}}
\newcommand{\Lti}     {L_{\mbox{\scriptsize ti}}}
\newcommand{\Lit}     {L_{\mbox{\scriptsize it}}}
\newcommand{\Ltt}     {L_{\mbox{\scriptsize tt}}}
\newcommand{\Lii}     {L_{\mbox{\scriptsize ii}}}
\newcommand{\Ldv}     {\mbox{{\sffamily L}}}
\newcommand{\Ltht}  {\textcolor{halfgreen}{{ \mbox{\lambdayb}_{\mbox{\hspace{-0.4em}\scriptsize t}} }}}   % translational thermal conductivity
\newcommand{\Lthi}  {\textcolor{halfgreen}{{ \mbox{\lambdayb}_{\mbox{\hspace{-0.4em}\scriptsize i}} }}}   % translational thermal conductivity

\newcommand{\ed}   {{i\delta}}  
\newcommand{\se}   {\displaystyle \sum_{i=1}^{n}}
\newcommand{\sd}   {\displaystyle \sum_{\delta=1}^{\ell_i}}
\newcommand{\sdi}  {\displaystyle \sum_{\delta=e,v,r}}
\newcommand{\sede} {\se\sd}

\newcommand{\mfe}  {m_{i}}                                    % component mass
\newcommand{\Ue}   {U_{i}}                                    % component internal energy
\newcommand{\Ued}  {U_{\ed}}                                         % dof       internal energy
\newcommand{\Se}   {S_{i}}                                    % component entropy
\newcommand{\Sed}  {S_{\ed}}                                         % dof       entropy
\newcommand{\Ted}  {T_{\ed}}                                         % dof       temperature
\newcommand{\Ter}  {T_{\epsilon\eta}}                                         % dof       temperature

\newcommand{\ssed} {\s^{\,\ast}_{\,\ed}}
\newcommand{\used} {u^{\ast}_{\ed}}

\newcommand{\lbar} {\bar{\ell}}
\newcommand{\lhat} {\hat{\ell}}

\newcommand{\ar}   {a=1,\cdots,n}                              % a range
\newcommand{\sa}   {\displaystyle \sum_{a=1}^{n}}
\newcommand{\sB}  {\displaystyle \sum_{b=1}^{n}}
\newcommand{\sbi}  {\displaystyle \sum_{b=1}^{n-1}}
\newcommand{\sC}  {\displaystyle \sum_{c=1}^{n}}
\newcommand{\RR} [1] {{\bv{R}}_{#1}}
\newcommand{\RP}  {\R_{\mbox{\tiny P}}}
\newcommand{\VP}  {\V_{\mbox{\tiny P}}}
\newcommand{\RRP}  {\RR{\mbox{\tiny P}}}
\newcommand{\RRd} [1] {  \dot{\bv{R}}_{#1}   }
\newcommand{\Rcm}    {{\bv{R}}_{\mbox{\tiny cm}}}
\newcommand{\Rcmd}    {\dot{\bv{R}}_{\mbox{\tiny cm}}}
\newcommand{\rr} [1] {{\bv{\mbox{$\frak{r}$}}}_{#1}}
\newcommand{\rrd} [1] {\dot{\bv{\mbox{$\frak{r}$}}}_{#1}}
\newcommand{\iv}{(\rr{},\rrd{})}
\newcommand{\dVc}{d^{3}\bv{c}}
\newcommand{\dViv}{(d^{3}\rr{}d^{3}\rrd{})}
\newcommand{\dVivg}{\textcolor{gray}{\dViv}}
\newcommand{\zodf}{f^{\mbox{\tiny (0)}}}
%\newcommand{\utr}{u_{\mbox{\tiny tr}}}
\newcommand{\ptr}{p_{\mbox{\tiny t}}}
\newcommand{\pin}{p_{\mbox{\tiny i}}}
\newcommand{\str}{s_{\mbox{\tiny t}}}
%\newcommand{\uin}{u_{\mbox{\tiny in}}}
\newcommand{\Sin}{s_{\mbox{\tiny i}}}
\newcommand{\Ztr}{Z_{\mbox{\tiny t}}}
%\newcommand{\Ttr}{T_{\mbox{\tiny tr}}}
\newcommand{\Zin}{Z_{\mbox{\tiny i}}}
%\newcommand{\Tin}{T_{\mbox{\tiny in}}}

==> myrgreekmacros.tex <==
% requires  rgreekmacros.tex; available only at 10pt (I believe)

\newcommand{\greekdg}[1]{\mbox{\begingreek#1\endgreek}}
\newcommand{\mgreekdg}[1]{\mbox{\beginmgreek#1\endmgreek}}

\newcommand{\alphay}{\mgreekdg{a}} 

\newcommand{\betay}{\mgreekdg{b}}

\newcommand{\gammay}{\mgreekdg{g}}

\newcommand{\deltay}{\mgreekdg{d}}
  \newcommand{\sdeltay}{\mgreekdg{\small d}}

\newcommand{\varepsilony}{\large \mgreekdg{e}}

\newcommand{\etay}{\mgreekdg{h}}
   \newcommand{\obetay}{\bar{\etay}}   % over-barred etay
   \newcommand{\setay}{\scalebox{0.80}{\etay}} % sub/superscript etay
   \newcommand{\etayA}{\etay_{\scalebox{0.5}{A}}}
%   \newcommand{\setayA}{\scalebox{0.825}{$\etayA$}} % sub/superscript etayA     
   \newcommand{\setayA}{{\setay}_{\scalebox{0.45}{A}}}
   \newcommand{\etayAa}{\etay_{\scalebox{0.5}{A,$a$}}}
   \newcommand{\setayAa}{{\setay}_{\scalebox{0.45}{A,$a$}}}
   \newcommand{\etayE}{\etay_{\scalebox{0.5}{E}}}
   \newcommand{\etayEa}{\etay_{\scalebox{0.5}{E,$a$}}}
   \newcommand{\etayK}{\etay_{\scalebox{0.5}{K}}}
   \newcommand{\etayKa}{\etay_{\scalebox{0.5}{K,$a$}}}

\newcommand{\thetay}{\mgreekdg{j}}

\newcommand{\iotay}{\mgreekdg{i}}

\newcommand{\ky}{\mgreekdg{k}}
   \newcommand{\kyb}{\mgreekdg{\bf k}}
   \newcommand{\kys}{\mgreekdg{\sl k}}

\newcommand{\lambday}{\mgreekdg{l}}
   \newcommand{\lambdayb}{\mgreekdg{\bf l}}
   \newcommand{\lambdays}{\mgreekdg{\sl l}}

\newcommand{\muy}{\mgreekdg{m}}
   \newcommand{\lmuy}{\mgreekdg{\large m}}
   \newcommand{\muyb}{\mgreekdg{\bf m}}

\newcommand{\nuy}{\mgreekdg{n}}

\newcommand{\xiy}{\mgreekdg{x}}
   \newcommand{\xiyA}{\xiy_{\scalebox{0.5}{A}}}
   \newcommand{\xiyE}{\xiy_{\scalebox{0.5}{E}}}
   \newcommand{\xiyK}{\xiy_{\scalebox{0.5}{K}}}
      
\newcommand{\piy}{\mgreekdg{p}}

\newcommand{\rhoy}{\mgreekdg{r}}
   \newcommand{\brhoy}{\bar{\rhoy}}
   \newcommand{\trhoy}{\tilde{\rhoy}}
   \newcommand{\trhoyA}{\tilde{\rhoy}_{\scalebox{0.5}{A}}}
   \newcommand{\trhoyE}{\tilde{\rhoy}_{\scalebox{0.5}{E}}}
   \newcommand{\trhoyK}{\tilde{\rhoy}_{\scalebox{0.5}{K}}}
   \newcommand{\rhoyc}{\rhoy_{\ssub{.6}{0}}}
   
\newcommand{\sigmay}{\mgreekdg{s}}
   \newcommand{\sigmayb}{\mgreekdg{\bf s}}

\newcommand{\tauy}{\mgreekdg{t}}

\newcommand{\phiy}{\mgreekdg{f}}

\newcommand{\psiy}{\mgreekdg{y}}


\newcommand{\Piy}{\mgreekdg{P}}
  \newcommand{\tPiy}{\tiny \mgreekdg{P}}

\newcommand{\Phiyb}{\mgreekdg{\bf F}}





==> rgreekmacros.tex <==
\def\lt{<}
\def\gt{>}
\newcount\fontnumber
\fontnumber=0
\newif\ifoneaccent\oneaccenttrue
\def\ifnextchar#1#2#3{\let\tempe #1\def\tempa{#2}\def\tempb{#3}\futurelet
  \tempc\ifnch}
\def\ifnch{\ifx\tempc\tempe\let\tempd\tempa\else\let\tempd\tempb\fi\tempd}
\def\gobble#1{}
\def\greekmode{%
\catcode`\<=13%
\catcode`\>=13%
\catcode`\'=11%
\catcode`\`=13%
\catcode`\~=11%
\catcode`\"=13%
\lccode`\<=`\<%
\lccode`\>=`\>%
\lccode`\'=`\'%
\lccode`\~=`\~%
\lccode`\"=`\"%
\def\rg{\fontnumber=1\tengr}%
\def\sl{\fontnumber=2\tengrsl}%
\def\it{\fontnumber=3\tengrit}%
\def\bf{\fontnumber=4\tengrbf}%
\def\smc{\fontnumber=5\tengrsmc}%
\def\I##1{\setbox0\hbox{##1}\ifdim\ht0=1ex\accent'174 ##1%
  \else{\ooalign{\hidewidth\char'174\hidewidth\crcr\unhbox0}}\fi}}%
\newcount\vwl
\newcount\acct
{
  \greekmode
  \gdef>{\ifnextchar ~{\expandafter\smoothcircumflex\gobble}{\char\lq\>}}
  \gdef<{\ifnextchar ~{\expandafter\roughcircumflex\gobble}{\char\lq\<}}
  \gdef\smoothcircumflex#1{\acct=\rq134 \vwl=\lq#1 \dobreathingcircumflex}
  \gdef\roughcircumflex#1{\acct=\rq100 \vwl=\lq#1 \dobreathingcircumflex}
  \gdef\dobreathingcircumflex{\ifnum\vwl\lt\rq140 %if uppercase
    \char\the\acct\kern -.2em\char\the\vwl\else
    \doaccent\fi}
  \gdef\doaccent{\accent\the\acct \char\the\vwl\relax}
  \gdef"{\ifnextchar '{\expandafter\diaeresisacute\gobble}{\accent\lq\"}}
  \gdef\diaeresisacute#1{\accent\rq043 #1}
  \gdef`{'}
}
 
\newif\ifgreek\greekfalse
 
\def\begingreek{\bgroup\font\tengr=rgrrg10\font\tengrsl=rgrsl10%
\font\tengrbf=rgrbf10\font\tengrit=rgrti10\font\tengrsmc=rgrsc10%
\greektrue\greekmode\rg}
\def\beginmgreek{\bgroup\font\tengr=mrgrrg10\font\tengrsl=mrgrsl10%
\font\tengrbf=mrgrbf10\font\tengrit=mrgrti10\font\tengrsmc=rgrsc10%
\greektrue\greekmode\rg}
\def\endgreek{\egroup}
\def\endmgreek{\egroup}
\def\monotoniko{%
\font\tengr=mrgrrg10\font\tengrsl=mrgrsl10%
\font\tengrbf=mrgrbf10\font\tengrit=mrgrti10%
\ifnum\fontnumber=5\smc%
  \else\ifnum\fontnumber=4\bf%
    \else\ifnum\fontnumber=3\it%
      \else\ifnum\fontnumber=2\sl%
        \else\rg%
      \fi%
    \fi%
  \fi%
\fi%
}
\def\polutoniko{%
\font\tengr=rgrrg10\font\tengrsl=rgrsl10%
\font\tengrbf=rgrbf10\font\tengrit=rgrti10%
\ifnum\fontnumber=5\smc%
  \else\ifnum\fontnumber=4\bf%
    \else\ifnum\fontnumber=3\it%
      \else\ifnum\fontnumber=2\sl%
        \else\rg%
      \fi%
    \fi%
  \fi%
\fi%
}
\let\math=$%
{\catcode`\$=13%
\gdef\greekdelims{\catcode`\$=13%
\def${\ifgreek\endgreek\else\begingreek\fi}
\def\display{\math\math}\def\enddisplay{\math\math}}}
\def\grave#1{{\edef\next{\the\font}\smc\accent\rq001\next#1}}
\def\roughgrave#1{{\edef\next{\the\font}\smc\accent\rq002\next#1}}
\def\smoothgrave#1{{\edef\next{\the\font}\smc\accent\rq003\next#1}}
\def\diaeresisgrave#1{{\edef\next{\the\font}\smc\accent\rq004\next#1}}
\def\diaeresiscircumflex#1{{\edef\next{\the\font}\smc\accent\rq005\next#1}}
\def\breve#1{{\edef\next{\the\font}\smc\accent\rq006\next#1}}
\def\macron#1{{\edef\next{\the\font}\smc\accent\rq007\next#1}}
\def\rhorough{{\tengrsmc
\ifnum\fontnumber=5\char\rq162
  \else\ifnum\fontnumber=4\char\rq016
    \else\ifnum\fontnumber=3\char\rq014
      \else\ifnum\fontnumber=2\char\rq012
        \else\char\rq010
      \fi
    \fi
  \fi
\fi
}}
\def\rhosmooth{{\tengrsmc
\ifnum\fontnumber=5\char\rq162
  \else\ifnum\fontnumber=4\char\rq017
    \else\ifnum\fontnumber=3\char\rq015
      \else\ifnum\fontnumber=2\char\rq013
        \else\char\rq011
      \fi
    \fi
  \fi
\fi
}}
\def\digamma{{\smc\char\rq135}}
\def\smallDigamma{{\smc\char\rq140}}
\def\Digamma{{\tengrsmc
\ifnum\fontnumber=5\char\rq021
  \else\ifnum\fontnumber=4\char\rq027
    \else\ifnum\fontnumber=3\char\rq025
      \else\ifnum\fontnumber=2\char\rq023
        \else\char\rq021
      \fi
    \fi
  \fi
\fi
}}
\def\vardigamma{{\tengrsmc
\ifnum\fontnumber=5\char\rq020
  \else\ifnum\fontnumber=4\char\rq026
    \else\ifnum\fontnumber=3\char\rq024
      \else\ifnum\fontnumber=2\char\rq022
        \else\char\rq020
      \fi
    \fi
  \fi
\fi
}}
\def\understroke{{\smc\char\rq046}}
\def\overstroke{{\smc\char\rq044}}
\def\sanpi{{\smc\char\rq136}}
\def\Sanpi{{\smc\char\rq137}}
\def\qoppa{{\smc\char\rq133}}
\def\varqoppa{{\smc\char\rq134}}
\def\Qoppa{{\smc\char\rq103}}
\def\Tao{{\smc\char\rq177}}
\def\ssh{\breve{s}}\def\SSH{\breve{S}}
\def\dz{\breve{z}}\def\DZ{\breve{Z}}
\def\psh{\breve{y}}\def\PSH{\breve{Y}}
\def\ksh{\breve{x}}\def\KSH{\breve{X}}
\def\inviota{{\smc\char\rq126}}
\def\grMF{{\smc\char\rq030\char\rq031\char\rq032\char\rq033}\-{\smc%
\char\rq034\char\rq036\char\rq037\char\rq032}}
\def\MF{{\smc\char\rq030\char\rq031\char\rq032\char\rq033}\-{\smc%
\char\rq040\char\rq036\char\rq037\char\rq032}}
 
\endinput
 

